Circumcentering the Douglas--Rachford method

We introduce and study a geometric modification of the Douglas-Rach\-ford method called the Circumcentered-Douglas-Rachford method. This method iterates by taking the intersection of bisectors of reflection steps for solving certain classes of feasibility problems. The convergence analysis is established for best approximation problems involving two (affine) subspaces and both our theoretical and numerical results compare favorably to the original Douglas-Rachford method. Under suitable conditions, it is shown that the linear rate of convergence of the Circumcentered-Douglas-Rachford method is at least the cosine of the Friedrichs angle between the (affine) subspaces, which is known to be the sharp rate for the Douglas-Rachford method. We also present a preliminary discussion on the Circumcentered-Douglas-Rachford method applied to the many set case and to examples featuring non-affine convex sets.

==> references.tex <==
%% Created using Papers on Tue, 18 Jul 2017.
%% http://papersapp.com/papers/

@article{Bauschke:1997wv,
author = {Bauschke, Heinz H and Borwein, Jonathan M and Lewis, A S},
title = {{The method of cyclic projections for closed convex sets in Hilbert space}},
journal = {Contemporary Mathematics},
year = {1997}
}

@article{Bauschke:2013jb,
author = {Bauschke, Heinz H and Luke, D Russell and Phan, Hung M and Wang, Xianfu},
title = {{Restricted Normal Cones and the Method of Alternating Projections: Theory}},
journal = {Set-Valued and Variational Analysis},
year = {2013},
volume = {21},
number = {3},
pages = {431--473},
month = may
}

@article{Douglas:1956kk,
author = {Douglas, Jim and Rachford, H H},
title = {{On the numerical solution of heat conduction problems in two and three space variables}},
journal = {Transactions of the American Mathematical Society},
year = {1956},
volume = {82},
number = {2},
pages = {421--421},
month = feb
}

@article{Phan:2016hl,
author = {Phan, Hung M},
title = {{Linear convergence of the Douglas{\textendash}Rachford method for two closed sets}},
journal = {Optimization},
year = {2016},
volume = {65},
number = {2},
pages = {369--385},
month = feb
}

@incollection{Deutsch:1995ja,
author = {Deutsch, Frank R},
title = {{The Angle Between Subspaces of a Hilbert Space}},
booktitle = {Approximation Theory, Wavelets and Applications},
year = {1995},
pages = {107--130},
publisher = {Springer Netherlands},
address = {Dordrecht}
}

@article{Bauschke:2015wf,
author = {Bauschke, Heinz H and Dao, Minh N and Noll, Dominikus and Phan, Hung M},
title = {{Proximal point algorithm, Douglas-Rachford algorithm and alternating projections: a case study}},
journal = {arXiv.org},
year = {2015},
eprint = {1501.06603v1},
eprinttype = {arxiv},
eprintclass = {math.OC},
month = jan
}

@article{Bezanson:2017gd,
author = {Bezanson, Jeff and Edelman, Alan and Karpinski, Stefan and Shah, Viral B},
title = {{Julia: A Fresh Approach to Numerical Computing}},
journal = {Siam Review},
year = {2017},
volume = {59},
number = {1},
pages = {65--98},
month = feb
}

@article{Knyazev:2006ek,
author = {Knyazev, Andrew V and Argentati, Merico E},
title = {{Principal Angles between Subspaces in an A-Based Scalar Product: Algorithms and Perturbation Estimates}},
journal = {SIAM Journal on Scientific Computing},
year = {2006},
volume = {23},
number = {6},
pages = {2008--2040},
month = jul
}

@article{Plesnik:2007ed,
author = {Plesn{\'\i}k, J{\'a}n},
title = {{Finding the orthogonal projection of a point onto an affine subspace}},
journal = {Linear Algebra and its Applications},
year = {2007},
volume = {422},
number = {2-3},
pages = {455--470},
month = apr
}

@article{Bjorck:1973jq,
author = {Bjorck, Ake and Golub, Gene Howard},
title = {{Numerical Methods for Computing Angles Between Linear Subspaces}},
journal = {Mathematics of Computation},
year = {1973},
volume = {27},
number = {123},
pages = {579},
month = jul
}

@article{Siqueira:2016ej,
author = {Siqueira, Abel Soares and da Silva, Raniere Costa and Santos, Luiz-Rafael},
title = {{Perprof-py: A Python Package for Performance Profile of Mathematical Optimization Software}},
journal = {Journal of Open Research Software},
year = {2016},
volume = {4},
number = {e12},
pages = {5},
month = apr
}

@article{Hesse:2014gi,
author = {Hesse, Robert and Luke, D Russell and Neumann, Patrick},
title = {{Alternating Projections and Douglas-Rachford for Sparse Affine Feasibility}},
journal = {IEEE Transactions on Signal Processing},
year = {2014},
volume = {62},
number = {18},
pages = {4868--4881},
month = jul
}

@article{ABTcomb,
author = {Arag{\'o}n Artacho, Francisco J and Borwein, Jonathan M and Tam, Matthew K},
title = {{Recent Results on Douglas{\textendash}Rachford Methods for Combinatorial Optimization Problems}},
journal = {Journal of Optimization Theory and Applications},
year = {2014},
volume = {163},
number = {1},
pages = {1--30}
}

@incollection{Boyle:1986do,
author = {Boyle, James P and Dykstra, Richard L},
title = {{A Method for Finding Projections onto the Intersection of Convex Sets in Hilbert Spaces}},
booktitle = {Advances in Order Restricted Statistical Inference},
year = {1986},
pages = {28--47},
publisher = {Springer New York},
address = {New York, NY}
}

@article{BCNPW14,
author = {Bauschke, Heinz H and Bello Cruz, Jose Yunier and Nghia, Tran T A and Phan, Hung M and Wang, Xianfu},
title = {{The rate of linear convergence of the Douglas{\textendash}Rachford algorithm for subspaces is the cosine of the Friedrichs angle}},
journal = {Journal of Approximation Theory},
year = {2014},
volume = {185},
pages = {63--79},
month = sep
}

@article{Lions:1979kk,
author = {Lions, P and Mercier, B},
title = {{Splitting Algorithms for the Sum of Two Nonlinear Operators}},
journal = {SIAM Journal on Numerical Analysis},
year = {1979},
volume = {16},
number = {6},
pages = {964--979},
month = dec
}

@article{Bauschke:2004fj,
author = {Bauschke, Heinz H and Combettes, Patrick L and Luke, D Russell},
title = {{Finding best approximation pairs relative to two closed convex sets in Hilbert spaces}},
journal = {Journal of Approximation Theory},
year = {2004},
volume = {127},
number = {2},
pages = {178--192},
month = apr
}

@incollection{Borwein:2011dq,
author = {Borwein, Jonathan M and Sims, Brailey},
title = {{The Douglas{\textendash}Rachford Algorithm in the Absence of Convexity}},
booktitle = {Fixed-Point Algorithms for Inverse Problems in Science and Engineering},
year = {2011},
pages = {93--109},
publisher = {Springer New York},
address = {New York, NY},
month = may
}

@article{Bauschke:2005ko,
author = {Bauschke, Heinz H and Combettes, Patrick L and Kruk, Serge G},
title = {{Extrapolation algorithm for affine-convex feasibility problems}},
journal = {Numerical Algorithms},
year = {2005},
volume = {41},
number = {3},
pages = {239--274},
month = dec
}

@article{Borwein:2014ka,
author = {Borwein, Jonathan M and Tam, Matthew K},
title = {{A Cyclic Douglas{\textendash}Rachford Iteration Scheme}},
journal = {Journal of Optimization Theory and Applications},
year = {2014},
volume = {160},
number = {1},
pages = {1--29}
}

@article{HernandezRamos:2011gf,
author = {Hern{\'a}ndez-Ramos, Luis M and Escalante, Ren{\'e} and Raydan, Marcos},
title = {{Unconstrained Optimization Techniques for the Acceleration of Alternating Projection Methods}},
journal = {Numerical Functional Analysis and Optimization},
year = {2011},
volume = {32},
number = {10},
pages = {1041--1066},
month = oct
}

@article{Dolan:2002du,
author = {Dolan, Elisabeth D and Mor{\'e}, Jorge J},
title = {{Benchmarking optimization software with performance profiles}},
journal = {Mathematical Programming},
year = {2002},
volume = {91},
number = {2},
pages = {201--213}
}

@article{Pang:2014dh,
author = {Pang, C H Jeffrey},
title = {{Set intersection problems: supporting hyperplanes and quadratic programming}},
journal = {Mathematical Programming},
year = {2014},
volume = {149},
number = {1-2},
pages = {329--359},
month = feb
}

@article{Pang:2013vf,
author = {Pang, C H Jeffrey},
title = {{Set intersection problems: Integrating projection and quadratic programming algorithms}},
journal = {arXiv.org},
year = {2013},
eprint = {1307.0053},
eprinttype = {arxiv},
month = jun
}

@article{Censor:2014gb,
author = {Censor, Yair and Cegielski, Andrzej},
title = {{Projection methods: an annotated bibliography of books and reviews}},
journal = {Optimization},
year = {2014},
volume = {64},
number = {11},
pages = {2343--2358},
month = oct
}

@article{benoist,
author = {Benoist, Jo{\"e}l},
title = {{The Douglas{\textendash}Rachford algorithm for the case of the sphere and the line}},
journal = {Journal of Global Optimization},
year = {2015},
volume = {63},
number = {2},
pages = {363--380},
month = may
}

@article{Pang:2014vr,
author = {Pang, C H Jeffrey},
title = {{Improved analysis of algorithms based on supporting halfspaces and quadratic programming for the convex intersection and feasibility problems}},
journal = {arXiv.org},
year = {2014},
eprint = {1406.4008},
eprinttype = {arxiv},
month = jun
}

@article{BCNPW15,
author = {Bauschke, Heinz H and Bello Cruz, Jose Yunier and Nghia, Tran T A and Phan, Hung M and Wang, Xianfu},
title = {{Optimal Rates of Linear Convergence of Relaxed Alternating Projections and Generalized Douglas-Rachford Methods for Two Subspaces}},
journal = {Numerical Algorithms},
year = {2016},
volume = {73},
number = {1},
pages = {33--76}
}

@article{Kayalar:1988jk,
author = {Kayalar, Selahattin and Weinert, Howard L},
title = {{Error bounds for the method of alternating projections}},
journal = {Mathematics of Control, Signals and Systems},
year = {1988},
volume = {1},
number = {1},
pages = {43--59}
}

@article{Bauschke:2015df,
author = {Bauschke, Heinz H and Noll, Dominikus and Phan, Hung M},
title = {{Linear and strong convergence of algorithms involving averaged nonexpansive operators}},
journal = {Journal of Mathematical Analysis and Applications},
year = {2015},
volume = {421},
number = {1},
pages = {1--20},
month = jan
}

@article{ABglobal,
author = {Artacho, Francisco J Arag{\'o}n and Borwein, Jonathan M},
title = {{Global convergence of a non-convex Douglas{\textendash}Rachford iteration}},
journal = {Journal of Global Optimization},
year = {2013},
volume = {57},
number = {3},
pages = {753--769}
}

@book{Deutsch:2001fl,
author = {Deutsch, Frank R},
title = {{Best Approximation in Inner Product Spaces}},
publisher = {Springer New York},
year = {2001},
series = {CMS Books in Mathematics},
address = {New York, NY}
}

@book{BC2011,
author = {Bauschke, Heinz H and Combettes, Patrick L},
title = {{Convex Analysis and Monotone Operator Theory in Hilbert Spaces}},
publisher = {Springer International Publishing},
year = {2017},
series = {CMS Books in Mathematics},
address = {Cham},
edition = {1}
}

@article{Bjorck:1973jqa,
author = {Bjorck, Ake and Golub, Gene Howard},
title = {{Numerical Methods for Computing Angles Between Linear Subspaces}},
journal = {Mathematics of Computation},
year = {1973},
volume = {27},
number = {123},
pages = {579},
month = jul
}

@article{Cimmino:1938tp,
author = {Cimmino, Gianfranco},
title = {{Calcolo approssimato per le soluzioni dei sistemi di equazioni lineari}},
journal = {La Ricerca Scientifica},
year = {1938},
volume = {9},
number = {II},
pages = {326--333}
}

@article{Borwein:2014co,
author = {Borwein, Jonathan M and Li, Guoyin and Yao, Liangjin},
title = {{Analysis of the Convergence Rate for the Cyclic Projection Algorithm Applied to Basic Semialgebraic Convex Sets}},
journal = {SIAM Journal on Optimization},
year = {2014},
volume = {24},
number = {1},
pages = {498--527},
month = jan
}

@incollection{Blanchini:2015ba,
author = {Blanchini, Franco and Miani, Stefano},
title = {{Set-theoretic estimation}},
booktitle = {Set-Theoretic Methods in Control},
year = {2015},
pages = {527--551},
publisher = {Springer International Publishing},
address = {Cham}
}

@article{Censor:2011hi,
author = {Censor, Yair and Chen, Wei and Combettes, Patrick L and Davidi, Ran and Herman, Gabor T},
title = {{On the effectiveness of projection methods for convex feasibility problems with linear inequality constraints}},
journal = {Computational Optimization and Applications},
year = {2011},
volume = {51},
number = {3},
pages = {1065--1088},
month = mar
}

@article{DePierro:1984ux,
author = {De Pierro, Alvaro Rodolfo and Iusem, Alfredo N},
title = {{A parallel projection method of finding a common point of a family of convex sets}},
journal = {Pesquisa Operacional},
year = {1984},
volume = {5},
number = {1},
pages = {1--20}
}

@article{Hesse:2013cv,
author = {Hesse, Robert and Luke, D Russell},
title = {{Nonconvex Notions of Regularity and Convergence of Fundamental Algorithms for Feasibility Problems}},
year = {2013},
volume = {23},
number = {4},
pages = {2397--2419},
month = jan
}

@article{Artacho:2014uo,
author = {Artacho, Francisco J Arag{\'o}n and Borwein, Jonathan M},
title = {{Recent Results on Douglas-Rachford Methods for Combinatorial Optimization Problems - ProQuest}},
journal = {Journal of Optimization {\ldots}},
year = {2014}
}

@article{Bozzo:1972ji,
author = {Bozzo, U and Tiramani, A R},
title = {{Tecniche di riordinamento delle equazioni per la risoluzione dei sistemi lineari sparsi}},
journal = {Calcolo},
year = {1972},
volume = {9},
number = {1-2},
pages = {139--142},
month = mar
}

@article{Combettes:1993dq,
author = {Combettes, P L},
title = {{The foundations of set theoretic estimation}},
journal = {Proceedings of the IEEE},
year = {1993},
volume = {81},
number = {2},
pages = {182--208},
month = feb
}

@manual{Feuersanger:2016ut,
title = {{PGFPlots Package}},
author = {Feuers{\"a}nger,  Christian},
edition = {1.13},
month = jun,
year = {2016}
}

@article{Bauschke:2006ej,
author = {Bauschke, Heinz H and Borwein, Jonathan M},
title = {{On Projection Algorithms for Solving Convex Feasibility Problems}},
journal = {Siam Review},
year = {2006},
volume = {38},
number = {3},
pages = {367--426},
month = jul
}

@article{ABT16,
author = {Arag{\'o}n Artacho, Francisco J and Borwein, Jonathan M and Tam, Matthew K},
title = {{Global behavior of the Douglas{\textendash}Rachford method for a nonconvex feasibility problem}},
journal = {Journal of Global Optimization},
year = {2016},
volume = {65},
number = {2},
pages = {309--327}
}

@article{Bauschke:2016bt,
author = {Bauschke, Heinz H and Moursi, Walaa M},
title = {{On the Douglas{\textendash}Rachford algorithm}},
journal = {Mathematical Programming},
year = {2016},
volume = {164},
number = {1-2},
pages = {263--284},
month = nov
}

@article{Gubin:1967ce,
author = {Gubin, L G and Polyak, B T and Raik, E V},
title = {{The method of projections for finding the common point of convex sets}},
journal = {USSR Computational Mathematics and Mathematical Physics},
year = {1967},
volume = {7},
number = {6},
pages = {1--24},
month = jan
}

@article{Iusem:1986bb,
author = {Iusem, Alfredo N and De Pierro, Alvaro Rodolfo},
title = {{Convergence results for an accelerated nonlinear cimmino algorithm}},
journal = {Numerische Mathematik},
year = {1986},
volume = {49},
number = {4},
pages = {367--378},
month = jul
}

@article{Bauschke:2003gb,
author = {Bauschke, Heinz H and Deutsch, Frank R and Hundal, Hein and Park, Sung-Ho},
title = {{Accelerating the Convergence of the Method of Alternating Projections}},
journal = {Transactions of the American Mathematical Society},
year = {2003},
volume = {355},
number = {9},
pages = {3433--3461},
month = sep
}

@book{Escalante:2011kf,
author = {Escalante, Ren{\'e} and Raydan, Marcos},
title = {{Alternating Projection Methods}},
publisher = {Society for Industrial and Applied Mathematics},
year = {2011},
series = {Fundamentals of Algorithms},
address = {Philadelphia, PA},
month = jan
}

@article{Svaiter:2011fb,
author = {Svaiter, Benar F},
title = {{On Weak Convergence of the Douglas{\textendash}Rachford Method}},
journal = {SIAM Journal on Control and Optimization},
year = {2011},
volume = {49},
number = {1},
pages = {280--287},
month = jan
}

@article{Birgin:2006bd,
author = {Birgin, Ernesto Giulian and Raydan, Marcos},
title = {{Robust Stopping Criteria for Dykstra's Algorithm}},
journal = {SIAM Journal on Scientific Computing},
year = {2006},
volume = {26},
number = {4},
pages = {1405--1414},
month = jul
}

@phdthesis{Tam:2012vp,
author = {Tam, Matthew K},
title = {{The Method of Alternating Projections}},
year = {2012},
address = {University of New Castle},
month = nov
}

@incollection{Deutsch:1985gz,
author = {Deutsch, Frank R},
title = {{Rate of Convergence of the Method of Alternating Projections}},
booktitle = {Parametric Optimization and Approximation: Conference Held at the Mathematisches Forschungsinstitut, Oberwolfach, October 16{\textendash}22, 1983},
year = {1985},
editor = {Brosowski, B and Deutsch, Frank R},
pages = {96--107},
publisher = {Birkh{\"a}user Basel},
address = {Basel}
}

@article{Gearhart:1989kw,
author = {Gearhart, William B and Koshy, Mathew},
title = {{Acceleration schemes for the method of alternating projections}},
journal = {Journal of Computational and Applied Mathematics},
year = {1989},
volume = {26},
number = {3},
pages = {235--249},
month = jul
}

@article{BNlocal,
author = {Bauschke, Heinz H and Noll, Dominikus},
title = {{On the local convergence of the Douglas{\textendash}Rachford algorithm}},
journal = {Archiv der Mathematik},
year = {2014},
volume = {102},
number = {6},
pages = {589--600}
}

@article{Ansorge:1984he,
author = {Ansorge, R},
title = {{Connections between the Cimmino-method and the Kaczmarz-method for the solution of singular and regular systems of equations}},
journal = {Computing},
year = {1984},
volume = {33},
number = {3-4},
pages = {367--375},
month = sep
}

@article{Drmac:2006er,
author = {Drmac, Zlatko},
title = {{On Principal Angles between Subspaces of Euclidean Space}},
journal = {SIAM Journal on Matrix Analysis and Applications},
year = {2006},
volume = {22},
number = {1},
pages = {173--194},
month = jul
}

@phdthesis{Tam:2016iw,
author = {Tam, Matthew K},
title = {{Iterative Projection and Reflection Methods: Theory and 
Practice 
}},
year = {2016},
address = {Newcastle},
month = may
}


